BASE: Probably a Better Approach to Multi-Object Tracking

The field of visual object tracking is dominated by methods that combine simple tracking algorithms and ad hoc schemes. Probabilistic tracking algorithms, which are leading in other fields, are surprisingly absent from the leaderboards. We found that accounting for distance in target kinematics, exploiting detector confidence and modelling non-uniform clutter characteristics is critical for a probabilistic tracker to work in visual tracking. Previous probabilistic methods fail to address most or all these aspects, which we believe is why they fall so far behind current state-of-the-art (SOTA) methods (there are no probabilistic trackers in the MOT17 top 100). To rekindle progress among probabilistic approaches, we propose a set of pragmatic models addressing these challenges, and demonstrate how they can be incorporated into a probabilistic framework. We present BASE (Bayesian Approximation Single-hypothesis Estimator), a simple, performant and easily extendible visual tracker, achieving state-of-the-art (SOTA) on MOT17 and MOT20, without using Re-Id. Code will be made available at https://github.com/ffi-no

==> figures/sht-fig.tex <==
\begin{figure*}
    \centering
    \begin{tikzpicture}[every text node part/.style={align=center}, font=\sffamily]
    \definecolor{graycolor}{HTML}{cccccc}
    \definecolor{redcolor}{HTML}{e06666}
    
    \draw[fill=graycolor] (-8, 3.5) rectangle (-4.5, 1) {};
    \node at (-8,3.5) [anchor=north west, inner sep=2mm] {Detector};
    
    \node at (-6.45,2.185) [draw, thick, minimum height=1.0cm, minimum width=2.1cm, fill=graycolor] {\small Detections};
    \node at (-6.25,1.985) [draw, thick, minimum height=1.0cm, minimum width=2.1cm, fill=graycolor] {\small Detections};
    \node at (-6.05,1.785) [draw, thick, minimum height=1.0cm, minimum width=2.1cm, fill=graycolor] {\small Detections};
    
    \node at (0,0) [draw, thick, minimum height=1.2cm, minimum width=3.4cm, rounded corners, fill=graycolor] {Track Management};
    
    \node at (3.0,1.485) [draw, thick, minimum height=1.2cm, minimum width=2.8cm, rounded corners, fill=graycolor] {Gating};
    
    \node at (7,1.485) [draw, thick, minimum height=1.2cm, minimum width=2.8cm, rounded corners, fill=graycolor] {Association};
    
    \node at (-2.75, -2.825) [draw, thick, minimum height=1.2cm, minimum width=2.5cm, rounded corners, fill=graycolor] {Predict};
    
    \node at (3, -2.825) [draw, thick, rounded corners=8pt, minimum height=1.8cm, minimum width=3.0cm] {};
    \node at (3, -2.40) [draw, thick, minimum height=0.6cm, minimum width=2.6cm, rounded corners, fill=graycolor] {\small Candidate tracks};
    \node at (3, -3.25) [draw, thick, minimum height=0.6cm, minimum width=2.6cm, rounded corners, fill=graycolor] {\small Tracks};
    
    \node at (6.2625, -2.4) [draw, thick, minimum height=0.6cm, minimum width=1.325cm, rounded corners, fill=graycolor] {\small Init};
    \node at (7.7375, -2.4) [draw, thick, minimum height=0.6cm, minimum width=1.325cm, rounded corners, fill=graycolor] {\small Update};
    
    \node at (7, -3.25) [draw, thick, minimum height=0.6cm, minimum width=2.8cm, rounded corners, fill=graycolor] {\small Report tracks};

    % detections ->
    \draw [thick, dotted, -Triangle] (-5.0, 1.785) -- (1.6, 1.785);
    
    % predict ->
    \draw [thick, -Triangle] (-2.75, -2.225) -- (-2.75, 1.185) -- (1.6, 1.185);
    
    % probabilistic track management ->
    \draw [thick, -Triangle] (1.7,  0.24) -- (3.24,  0.24) -- (3.24, -2.10);
    \draw [thick, -Triangle] (1.7, -0.24) -- (2.76, -0.24) -- (2.76, -1.90);
    \node at (3.24,-1.12) [anchor=west, inner xsep=2mm] {Promote};
    \node at (2.76,-1.12) [anchor=east, inner xsep=2mm] {Kill};
    
    % probabilistic gating ->
    \draw [thick, dotted, -Triangle] (4.4, 1.785) -- (5.6, 1.785);
    \draw [thick, -Triangle] (4.4, 1.185) -- (5.6, 1.185);
    
    % probabilistic association ->
    \draw [thick, dotted, -Triangle] (6.4125, 0.885) -- (6.4125, -2.1);
    \draw [thick, -Triangle] (7.5875, 0.885) -- (7.5875, -2.1);
    \draw [thick, dotted, -Triangle] (7.8875, 0.885) -- (7.8875, -2.1);
    
    % init ->
    \draw [thick, -Triangle] (5.6, -2.4) -- (4.3,  -2.4);
    
    % update ->
    \draw [thick, -Triangle] (7.7375, -2.7) -- (7.7375, -2.825) -- (4.5,  -2.825);

    % tracks ->
    \draw [thick, -Triangle] (1.5,  -2.825) -- (-1.5, -2.825);
    \draw [thick, -Triangle] (4.3,  -3.25) -- (5.6, -3.25);
    
    \end{tikzpicture}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}



==> figures/tracktor-fig.tex <==
\begin{figure*}
    \centering
    \begin{tikzpicture}[every text node part/.style={align=center}, font=\sffamily]
    \definecolor{graycolor}{HTML}{cccccc}
    \definecolor{redcolor}{HTML}{e06666}
    
    \draw[fill=graycolor] (-8, 3.5) rectangle (-4.5, -0.815) {};
    \node at (-8,3.5) [anchor=north west, inner sep=2mm] {Detector};
    
    \node at (-6.45,2.185) [draw, thick, minimum height=1.0cm, minimum width=2.1cm, fill=graycolor] {\small Detections};
    \node at (-6.25,1.985) [draw, thick, minimum height=1.0cm, minimum width=2.1cm, fill=graycolor] {\small Detections};
    \node at (-6.05,1.785) [draw, thick, minimum height=1.0cm, minimum width=2.1cm, fill=graycolor] {\small Detections};
    
    \node at (0,0) [draw, thick, minimum height=1.2cm, minimum width=3.4cm, rounded corners, fill=redcolor] {Probabilistic\\Track Management};
    
    \node at (3.0,1.485) [draw, thick, minimum height=1.2cm, minimum width=2.8cm, rounded corners, fill=redcolor] {Probabilistic\\Gating};
    
    \node at (7,1.485) [draw, thick, minimum height=1.2cm, minimum width=2.8cm, rounded corners, fill=redcolor] {Probabilistic\\Association};
    
    \node at (-6.25,-0.24) [draw, thick, minimum height=2.45cm, minimum width=3.1cm] {};
    \node at (-6.25,0.335) [draw, thick, minimum height=1.0cm, minimum width=2.8cm, fill=redcolor] {\small Clutter model};
    \node at (-6.25,-0.815) [draw, thick, minimum height=1.0cm, minimum width=2.8cm, fill=redcolor] {\small Target birth model};
    
    \node at (-2.75, -2.825) [draw, thick, minimum height=1.2cm, minimum width=2.5cm, rounded corners, fill=graycolor] {Predict};
    
    \node at (3, -2.825) [draw, thick, rounded corners=8pt, minimum height=1.8cm, minimum width=3.0cm] {};
    \node at (3, -2.40) [draw, thick, minimum height=0.6cm, minimum width=2.6cm, rounded corners, fill=graycolor] {\small Candidate tracks};
    \node at (3, -3.25) [draw, thick, minimum height=0.6cm, minimum width=2.6cm, rounded corners, fill=graycolor] {\small Tracks};
    
    \node at (6.2625, -2.4) [draw, thick, minimum height=0.6cm, minimum width=1.325cm, rounded corners, fill=graycolor] {\small Init};
    \node at (7.7375, -2.4) [draw, thick, minimum height=0.6cm, minimum width=1.325cm, rounded corners, fill=graycolor] {\small Update};
    
    \node at (7, -3.25) [draw, thick, minimum height=0.6cm, minimum width=2.8cm, rounded corners, fill=graycolor] {\small Report tracks};

    % clutter model, target birth model ->
    \draw [thick, dashed, -Triangle] (-4.7, -0.24) -- (-1.7, -0.24);
    \draw [thick, dashed, -Triangle] (-3.7, -0.24) -- (-3.7, 1.485) -- (1.6, 1.485);
    
    % detections ->
    \draw [thick, dotted, -Triangle] (-5.0, 1.785) -- (1.6, 1.785);
    
    % predict ->
    \draw [thick, -Triangle] (-2.75, -2.225) -- (-2.75, 1.185) -- (1.6, 1.185);
    \draw [thick, -Triangle] (-2.75, 0.24) -- (-1.7, 0.24);
    
    % probabilistic track management ->
    \draw [thick, -Triangle] (1.7,  0.24) -- (3.24,  0.24) -- (3.24, -2.10);
    \draw [thick, -Triangle] (1.7, -0.24) -- (2.76, -0.24) -- (2.76, -1.90);
    \node at (3.24,-1.12) [anchor=west, inner xsep=2mm] {Promote};
    \node at (2.76,-1.12) [anchor=east, inner xsep=2mm] {Kill};
    
    % probabilistic gating ->
    \draw [thick, dotted, -Triangle] (4.4, 1.785) -- (5.6, 1.785);
    \draw [thick, dashed, -Triangle] (4.4, 1.485) -- (5.6, 1.485);
    \draw [thick, -Triangle] (4.4, 1.185) -- (5.6, 1.185);
    
    % probabilistic association ->
    \draw [thick, dashed, -Triangle] (6.1125, 0.885) -- (6.1125, -2.1);
    \draw [thick, dotted, -Triangle] (6.4125, 0.885) -- (6.4125, -2.1);
    \draw [thick, -Triangle] (7.5875, 0.885) -- (7.5875, -2.1);
    \draw [thick, dotted, -Triangle] (7.8875, 0.885) -- (7.8875, -2.1);
    
    % init ->
    \draw [thick, -Triangle] (5.6, -2.4) -- (4.3,  -2.4);
    
    % update ->
    \draw [thick, -Triangle] (7.7375, -2.7) -- (7.7375, -2.825) -- (4.5,  -2.825);

    % tracks ->
    \draw [thick, -Triangle] (1.5,  -2.825) -- (-1.5, -2.825);
    \draw [thick, -Triangle] (4.3,  -3.25) -- (5.6, -3.25);
    
    \end{tikzpicture}
    \caption{Tracktor-ish}
    \label{fig:tracktor-overview}
\end{figure*}


==> tex/88_litterature_stuff.tex <==
\section{Loosely written litterature stuff}

\subsection{Stuff we have to cite}

Your detector is based on the YOLOX modification from\cite{Zhang2021ByteTrack:Box}, and our videostabilization is based on BoT-SORT\cite{Aharon2022BoT-SORT:Tracking}

\subsection{About the other trackers}

\subsubsection{Bot-SORT \cite{Aharon2022BoT-SORT:Tracking}}

BoT-SORT introduces new ideas into ByteTrack. \textit{In this work, we propose new trackers which outperform
all leading trackers in all the main MOT metrics (Figure 1) for the MOT17 and MOT20 challenges, by addressing the above SORT-like tracker’s limitations and integrating them into the novel ByteTrack}
Novelties
\begin{itemize}
    \item Camera-compensation
    \item Kalman filter state vector
\end{itemize}

\subsubsection{FOR-Tracking}
They have made some evaluations as to the performance of the detector:
\begin{figure}[H]
    \includegraphics{"figures/tmp_litterature_review/for_tracking_accumulative_tp_fp.png"}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
Novelties:
\begin{itemize}
    \item Novel interaction cue based on geometric features
    \item Camera motion estimation based on the tracker itself
    \item Similiraty metric based on detection size?
\end{itemize}
Association: Dual-threshold, cascade. Combination of motion and appearence AND interaction. 
Lower similarty demand in first step. 
Uses normalized IOU - 
States: center, aspect, height and their derivatives



Based on: ``Simple online and real-time tracking with occlusion handling``


\subsubsection{Quo-Vadis}
Based on bytetrack, the primary goal to be able to bridge long occlusions. 

They use a depth-estimation and segmentation to generate a BEV of the world and use forecasting models to generate hypothesis. 
Very minor improvement on MOT17. 6

\subsubsection{Tracking game}
Tracking game uses a self-adaptive agent tracker framework to solve the MOT tracking challenge. They use YOLOX to extract detections for the agent 


\subsubsection{MAA-track}
MAA-track uses a uses a special association method for the tracks that are close together. 
They had some kind of intersting findings. 

If there are two confused tracks, the most effective approach for their tracker is to delete the detection they are fighting for and simply propagate the tracks until they are well-separated again. 

They have also modified the interpolation to include camera motion. 
They do not estimate the size of the bounding box during occlusions, but simply propagate it.

Their "winning" submission uses CrowdDet as a detector. 
For the ambiguous situations, they delete detections if there are more tracks than detections and use candidate-tracks if there are more detections then tracks. 
For the interpolation they use motion-aware interpolation and height-preservation for the bounding boxes. 

\subsubsection{MO3TR}
`Looking beyound two frames: End-to-end multi-object tracking using spatial and temporal transformers. 

A very intersting paper that should be read in detail just for fun, but to this paper, the primary points are: 
- end-to-end transformer based tracker. 


\subsubsection{MOTR}
Same as above

\subsubsection{OC-SORT}
`Observation-Centric SORT: Rethinking SORT for robust multi-object tracking`
The main idea behing OC-SORT is to value the observations more than the estimation (KF). The approach is based on SORT, but claims that SORT is inaccurate in three main areas:
\begin{itemize}
    \item The noise of the detections is in the order of magnitude of the relative displacement between frames, leading to large variance in KF velocity estimate
    \item The state noise is again made worse when objects are occluded
    \item Desire to make SORT observation-centric and not estimation-centric
\end{itemize}

These three limitations are addressed by three innovations:
\begin{itemize}
    \item Observation-centric online smooting: When a track is found after being occluded, and a virtual trajectory to that point from last observation is made. The KF parameters are then smoothed according to that trajectory. 
    \item Incorporating direction consistency in the track-comparison scoring
    \item Observation-centric recovery
\end{itemize}

\subsubsection{Re-MOT}
Essentially an offline refinement stage.
A semi self-supervised approach to refine tracking results. 
Not really a tracker per-se.

\subsubsection{CorrTracker}
`Multiple object tracking with correlation learning`
CVPR 2021
Based on FairMOT, has a pretty nice organization of the litterature review. 
Centernet detector. 
Corrtracker is:
\begin{itemize}
    \item CorrTracker, a unified correlation trackerto intensively model associations between objects andtransmit information through associations.• We propose a local structure-aware network and en-hance the discriminability of similar objects with self-supervised learning.
    \item We extend the local correlation network to model temporal information efficiently.
    \item CorrTracker shows significant improvements over ex-isting state-of-the-art results in four MOT benchmarks.In particular, we achieve76.5%MOTA and IDF1 of73.6%on MOT17.
\end{itemize}

\subsubsection{FairMOT}


\subsubsection{JDE}

\subsubsection{Unicorn}
`towards grand unification of object tracking`
Single model end-to-end SOT, MOT, VOS and MOTS. 

\subsubsection{Permatrack}
`Learning to track with object permanence`. 

Builds on top of Centertrack, but extends the memory module to focus on the objects that are permanent. End-to-end joint detection and tracking. 

\subsubsection{Strong-SORT}
Further improvements on Deep-SORT by:
\begin{itemize}
    \item Replacing the cnn re-id module with BoT
    \item Replacing the standard kalman-filter with NSA-kalman filter
    \item Replace matching pyramid with global linear assignment
    \item Replace the detector with YOLO-X
    \item They use GPR/GSI instead of CMC(VO)
\end{itemize}

From the ablation:
\begin{itemize}
    \item BoT -> Improvements in IDF1
    \item ECC -> VO improves IDF1
    \item NSA -> improves HOTA
    
\end{itemize}

\subsubsection{Center-track}

\subsubsection{SORT}
`Simple Online and Realtime Tracking`

Identifies detection quality as a key factor for track-quality. 

SORT is indeed a simple and online tracker. 
It incorporates a kalmanfilter for the state of the tracks and IOU as the only matching strategy. They also use candidate tracks (or probation as they call it). 
However, it is a very naive approach, much because \verb#t_lost# is 1, meaning that is cannot handle any faults in the detector or occluded objects. 
\subsubsection{Deep-SORT}
Essentially the same as SORT, but with appearance as well, but they also introduce the infamous matching-cascade. The addition of appearance makes the able to make \verb#t_lost# or \verb#a_max# as they call it a lot larger, close to 30 frames. 
The performance of the original SORT with the same detections was 59.8, including deep features increases the MOTA to 61.4. 

The motivation for the matching cascade was to counteract the fact that old tracks get a large uncertanty and hence matching in mahalanobis distance makes them "prioritized" in matching. Therefore, the cascade starts with the newly-observed tracks and works it way down, favouring newly observed tracks. 

No VO was added. 

\subsubsection{Giaotracker}


\subsubsection{Multi-Level Cooperative Fusion of GM-PHD Filters for Online Multiple Human Tracking}
They use an GM-PHD implementation to fuse public detections with their own body-part detector to "generate detections" where people are missed in the original detections. 
The goal of the fusion 

\label{sec:conclusione}

Vi gjør det spesielt bra på små objekter. Det er fordi hvert track får varierende grad konfidens av hver måling, så vi kan bruke lang tid på å etablere små tracks.
